Multi-Modal Fusion Transformer for Visual Question Answering in Remote Sensing

With the new generation of satellite technologies, the archives of remote sensing (RS) images are growing very fast. To make the intrinsic information of each RS image easily accessible, visual question answering (VQA) has been introduced in RS. VQA allows a user to formulate a free-form question concerning the content of RS images to extract generic information. It has been shown that the fusion of the input modalities (i.e., image and text) is crucial for the performance of VQA systems. Most of the current fusion approaches use modality-specific representations in their fusion modules instead of joint representation learning. However, to discover the underlying relation between both the image and question modality, the model is required to learn the joint representation instead of simply combining (e.g., concatenating, adding, or multiplying) the modality-specific representations. We propose a multi-modal transformer-based architecture to overcome this issue. Our proposed architecture consists of three main modules: i) the feature extraction module for extracting the modality-specific features; ii) the fusion module, which leverages a user-defined number of multi-modal transformer layers of the VisualBERT model (VB); and iii) the classification module to obtain the answer. Experimental results obtained on the RSVQAxBEN and RSVQA-LR datasets (which are made up of RGB bands of Sentinel-2 images) demonstrate the effectiveness of VBFusion for VQA tasks in RS. To analyze the importance of using other spectral bands for the description of the complex content of RS images in the framework of VQA, we extend the RSVQAxBEN dataset to include all the spectral bands of Sentinel-2 images with 10m and 20m spatial resolution.

==> old_sections/conclusion.tex <==
This study presents a novel architecture in RS VQA that applies a transformer model, which exclusively relies on multi-modal transformer layers, instead of a mixture of single and multi-modal layers, to jointly learn the image and text representation.
Our proposed architecture includes: i) a feature extraction module base on the BoxExtractor and the BertTokenizer; ii) a fusion module based on x multi-modal transformer layers of VisualBERT; and iii) a classification module consisting of an \gls{mlp} projection head.
To show the effectiveness, we evaluated the model on the RGB RSVQAxBEN (which includes only RGB bands of Sentinel-2 tiles), the 10B RSVQAxBEN (which includes 10 bands), and the RSVQA LR dataset.
We show a notable performance increase for the large-scale RGB RSVQAxBEN dataset compared to a non-learnable fusion module.
Increasing the size and depth of the transformer leads to further performance gains.
% The performance increase of our method becomes even higher if we take more VisualBERT layer.
A noteworthy result is the slight performance difference between our general model and the more specialized Prompt-RSVQA.
In contrast to the results on the large-scale RSVQAxBEN dataset, we could only show a slight performance increase for the comparably small RSVQA LR dataset compared to the SkipRes architecture, which utilizes a simple static fusion module.
Compared to the relatively large complexity of our models, the slight improvement aligns with the literature findings that big transformers struggle on small datasets.
% Compared to the relatively large complexity of our models, the small improvement 
% TODO: come up with a better sentence about transformer!
In addition, we cannot see a significant improvement in the dataset with larger layer configurations.
Our results show that our general multi-modal transformer-based fusion module requires larger datasets to realize its full potential.
% Our results show that our proposed multi-modal transformer-based fusion module is able to improve the performance of VQA models with
%However, regarding the big RS image archives there are large-scale datasets available.
% However, with the ever-increasing remote sensing archives, the sizes of future datasets are expected to increase.
% Requires a lot data <= Ok because RS a lot of data
Finally, when using 10B RSVQAxBEN, even the smallest model (VB4Fusion) outperforms SkipRes (trained on RGB) by more than 5\% in global accuracy and slightly beats VB12Fusion trained on RGB. 
It is worth noting that our architecture is not limited to specific questions, e.g. questions concerning pre-defined objects.
% Kai: check again later

Although transformer-based models have a high potential to improve the performance in RS VQA, future work may include research with smaller models and fusion modules on smaller datasets, such as RSVQA LR dataset.
These smaller models can then be analyzed on RSVQAxBEN (RGB and 10B) and compared with larger transformers to investigate the trade-off between complexity and performance.
In addition, pre-training of these transformer architectures may be necessary for high-performing RS VQA models.
This necessity is based on the observation that the performance jumps for LC accuracy when we utilize all pre-trained layers (VB12Fusion) on the RGB RSVQAxBEN and just slightly improves (compared to the other VBxFusion models) the performance on the 10B RSVQAxBEN dataset.
Furthermore, we are planning complementary research that will extend our feature extraction module to optimize the BoxExtractor or exchange it with a more sophisticated general box extractor.
As a final remark, we would like to note that the RSVQAxBEN dataset has to overcome the limitations of simple LC-based questions.
It would be beneficial to utilize the recommended 19-class nomenclature of BigEarthNet as the class label basis.
This upgrade should include complex questions, such as relationship and area-based questions.
Finally, more research should investigate the importance of multispectral information for RS VQA, using the available 10B RSVQAxBEN.


==> old_sections/experiments.tex <==
We conducted experiments on the RSVQA LR\citenum{RSVQA} and the RSVQAxBEN\citenum{RSVQAxBEN} datasets.
The RSVQA LR dataset was constructed using 7 Sentinel-2 tiles acquired over the Netherlands, from which only the RGB bands were used.
The tiles are divided into 772 patches of size 256x256 pixels.
To obtain the information needed to create the image-question-answer triplets, knowledge from the publicly available OpenStreetMap database was leveraged.
With this knowledge, the dataset was constructed by taking an image patch and randomly building question-answer pairs from a given template.
This procedure resulted in 77,232 image-question-answer triplets.
As in \citenum{RSVQA}, we used the same tile-based train/validation/test split.
The training split consists of five tiles, whereas the validation and test split consist of one tile each. 
For further information on the RSVQA LR dataset (e.g., the definition of the question classes), the reader is referred to \citenum{RSVQA}.

The large-scale RSVQAxBEN\citenum{RSVQAxBEN} dataset embodies the largest freely available RS VQA dataset.
It is based on the BigEarthNet\citenum{BEN} (BEN) archive and contains 590,326 different Sentinel-2 image patches, each covering an area of 1200m\,x\,1200m.
These image patches have spectral bands of varying resolutions.
Concretely, there are bands with three different resolutions: 10m, 20m, and 60m, resulting in 120x120, 60x60, and 20x20 pixels per image.
The Sentinel-2 tile originally contained 13 bands, but since band B10 contains no surface-level information, it was dropped after calculating the bottom-of-atmosphere reflectance values, resulting in patches with 12 spectral channels.
The content of each patch is described by multiple class labels from the CORINE Land Cover (CLC) 2018 database. 
The CLC class labels are categorized into three hierarchical groups.
The first group (L1) contains the most coarse labels, such as agricultural areas.
In the second (L2) and third (L3) groups, the included classes become more specific, such as arable land (L2) and non-irrigated arable land (L3).
The RSVQAxBEN dataset was constructed as a large-scale benchmark for RS VQA, using only the RGB bands of the BEN patches.
A stochastic algorithm that utilizes the CLC labels produced the image question-answer triplets.
% A stochastic algorithm, that took advantage of the CLC labels, produced the image-question-answer triplets.
The procedure described in \citenum{RSVQAxBEN} resulted in 14,758,150 image-question-answer triplets, which include 26,875 unique answers.
To limit the number of possible answers, the model's output in \citenum{RSVQAxBEN} was restricted to the 1,000 most frequent answers, covering 98.1\% of the answer set.
For the sake of comparability, we also apply this restriction.
We use the same train/validation/test split based on the tiles' spatial location as in \citenum{RSVQAxBEN}.
For more statistical insights, the reader is referred to  \citenum{RSVQAxBEN}\,.

We provide experimental results on the original RSVQAxBEN dataset. 
In addition, we extend the original three-band RSVQAxBEN dataset to a ten-band version.
We chose the 10m (B02, B03, B04, B08) and 20m (B05, B06, B07, B8A, B11, B12) bands for our experiments, where we interpolated the 20m bands to the resolution of the 10m bands.
The 60m bands (B01, B09) were not used because of their low-spatial resolution and their main application being water vapor and cirrus cloud detection.
To differentiate between the three- and ten-band dataset variants, we named them RGB and 10B RSVQAxBEN, respectively.
% interpolate

We performed our experiments with different layer configurations for our proposed VBxFusion architecture given by the VisualBERT\citenum{VisualBERT} model. 
We selected five configurations, where x $\in\{4, 6, 8, 10, 12\}$ in VBxFusion, defines the corresponding number of layers selected from the original VisualBERT model.
Note that VB12Fusion is identical to the original VisualBERT model.
As an initialization, we have chosen the weights pre-trained on ImageNet\citenum{ImageNet}\,. 
% Note that the VisualBERT model is pre-trained on ImageNet\cite{ImageNet}\,.\todo{maybe rewrite}
% We will also select the layers for the smaller models from these pre-trained layers. % <- In my opinion this is more confusing than helpful. The previous sentence implies that we use the pretrained weights and 12 layers are the full layers
For the RSVQA LR and RGB RSVQAxBEN datasets, we extracted ten boxes, and for 10B RSVQAxBEN we extracted five boxes. 
The learning rate was set to $10^{-6}$, the maximum number of training epochs was 300 for RSVQA LR and 15 for RSVQAxBEN, and we chose a batch size of 1024 and 2048, respectively.
The runs were performed on an NVIDIA A100-SXM4-80GB.
We used the implementation from the Huggingface library\citenum{wolf-etal-2020-transformers} for the VisualBERT layers.
Our architecture was compared with the SkipRes\citenum{RSVQA,RSVQAxBEN} (based on Skip-Thoughts and ResNet152), CrossModal \citenum{cross-modal}, and Prompt-RSVQA \citenum{Chappuis_2022_CVPR} results from the respective papers.
To analyze the results on the RSVQA LR we consider the accuracy's per question type.
These accuracy's are named \enquote{Count}, \enquote{Presence}, \enquote{Comparison} and \enquote{Rural/Urban}.
Further, we provide the average over the question type accuracy's and the overall accuracy, denoted as \enquote{AA} and \enquote{OA}.
The metrics used to analyze the results on the RSVQAxBEN dataset are given by: \enquote{Global}, which denotes the overall accuracy, as well as \enquote{Yes/No} and \enquote{LC}, which denotes the accuracy of the corresponding question types.
Notice that we use the same names of the metrics as in the respective papers.


\begin{table}[tb!]
    \centering
    \caption{Accuracies obtained by using different VQA models on the RSVQA LR Dataset. Bold values highlight the best and underlined values the second best accuracy.}
    \begin{tabular}{l K K K K K K}
    \toprule
    {Model} & {Count} & {Presence} & {Comparison} & {Rural/Urban} & {AA} & {OA} \\
    \midrule
    SkipRes & 67.01 & 87.46 & 81.50 & \textbf{90.00} & 79.08 & 81.49 \\
    VB4Fusion & 68.17 & 88.02 & 88.51 & 87.00 & 82.92 & 82.36 \\
    VB6Fusion & 68.17 & 88.87 & \underline{88.83} & 84.00 & 82.47 & 82.71 \\
    VB8Fusion & \underline{69.36} & 89.00 & 83.46 & \underline{88.00} & 82.45 & 80.99 \\
    VB10Fusion & 67.73 & \underline{89.48} & 86.68 & \underline{88.00} & \textbf{82.97} & 81.94  \\
    VB12Fusion & 68.14 & 89.27 & 88.71 & 85.00 & \underline{82.78} & \underline{82.78} \\
    CrossModal & \textbf{70.06} & \textbf{91.85} & \textbf{93.07} & 50.00 & 76.21 & \textbf{85.50} \\
    \bottomrule
    \end{tabular}
    \label{RSVQA_LR_acc}
\end{table}
% \begin{table}[tb!]
%     \centering
%     \caption{Accuracy obtained by the different models on the RSVQA LR Dataset.}
%     \begin{tabularx}{\linewidth}{l X X X X X X}
%     \toprule
%     Model & Count & Presence & Comparison & Rural/Urban & AA & OA \\
%     \midrule
%     SkipRes & 67.01 & 87.46 & 81.50 & 90.00 & 79.08 & 81.49 \\
%     VB4layer & 68.17 & 88.02 & 88.51 & 87.00 & 82.92 & 82.36 \\
%     VB6layer & 68.17 & 88.87 & 88.83 & 84.00 & 82.47 & 82.71 \\
%     VB8layer & 69.36 & 89.00 & 83.46 & 88.00 & 82.45 & 80.99 \\
%     VB10layer & 67.73 & 89.48 & 86.68 & 88.00 & 82.97 & 81.94  \\
%     VB12layer & 68.14 & 89.27 & 88.71 & 85.00 & 82.78 & 82.78 \\
%     CrossModal & 70.06 & 91.85 & 93.07 & 50.00 & 76.21 & 85.50 \\
%     \bottomrule
%     \end{tabularx}
%     \label{RSVQA_LR_acc}
% \end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experimental Results}\label{sec:experimental_results}

The results of the RSVQA LR dataset are presented in \cref{RSVQA_LR_acc}.
By analyzing the tables, one can see that our proposed VBxFusion models significantly outperform the SkipRes model in AA, whereas our models are just slightly better in OA.
The most significant difference occurs in the \enquote{Comparison} accuracy, which represents the most challenging question type. 
Here, a model is required to count the number of occurrences of a selected object with a specific positional relationship to a reference object.
Furthermore, no significant improvement is observed when increasing the number of VisualBert layers. 
% Compared to the relatively large complexity of our models, the slight improvement is aligned with the common knowledge that big transformers\cite{VIT} struggle on small datasets.
Compared to the relatively large complexity of our models, the slight improvement aligns with the findings of \citenum{VIT} that large transformers struggle on small datasets.
In the case of the \enquote{Rural/Urban} questions, the under performance can be explained with the same argument; there are too few questions of this type.
This is because the \enquote{Rural/Urban} question type makes up the smallest proportion of the dataset (1\%).

% The Rural/Urban question-type is the smallest question type that only takes up 1\% of the dataset.
When comparing our results to CrossModal, our model underperforms in OA because most questions are concerned with predictable objects.
However, our model has a higher AA score, which underlines the general characteristics of our proposed architecture.


The results for the RGB RSVQAxBEN dataset are presented in \cref{RGB_RSVQAxBEN_acc}. 
We see that even the smallest VBxFusion model outperforms the SkipRes model in terms of Global accuracy, and the performance increases if we utilize more VisualBERT layers.
Interestingly, we see that the VB12Fusion model's performance jumps in LC accuracy.
A possible explanation is that the VB12Fusion utilizes all pre-trained layers instead of partially rejecting layers.
Therefore, the initial weights can produce more meaningful embeddings than the pruned models.
Furthermore, the comparison shows that our model is competitive with the Prompt-RSVQA\citenum{Chappuis_2022_CVPR} model.
This highlights the effectiveness of our architecture since we are not exploiting the structure of the dataset.

\begin{table}[t!]
    \caption{Accuracies obtained using different VQA models on the (a) RGB and (b) 10B RSVQAxBEN dataset. Bold values highlight the best and underlined values the second best accuracy.}
    \vspace{1em}
    \begin{subtable}[t]{.44\linewidth}
    \caption{Results on RGB RSVQAxBEN}
    \begin{tabular*}{\linewidth}{l @{\extracolsep{\fill}} K K K }
    \toprule
    {Model} & {Global} & {Yes/No} & {LC} \\
    \midrule
    SkipRes & 69.92 & 80.02 & 20.68 \\
    VB4Fusion & 73.06 & 83.86& 20.40  \\
    VB6Fusion & 73.88 & 84.58 & 21.66 \\
    VB8Fusion & 73.43 & 84.37 & 20.07 \\
    VB10Fusion & 74.19 & 85.13 & 20.82 \\
    VB12Fusion & \underline{75.07} & \underline{85.47} & \underline{24.33} \\
    Prompt-RSVQA & \textbf{75.40} & \textbf{86.07} & \textbf{26.56} \\
    \bottomrule
    \end{tabular*}
    \label{RGB_RSVQAxBEN_acc}
    \end{subtable}\hfill
    \begin{subtable}[t]{.44\linewidth}
    \centering
    \caption{Results on 10B RSVQAxBEN}
    \begin{tabular*}{\linewidth}{l @{\extracolsep{\fill}} K K K}
    \toprule
    {Model} & {Global} & {Yes/No} & {LC} \\
    \midrule
    VB4Fusion  & 75.26 & 85.41 & 25.72 \\
    VB6Fusion  & 75.34 & 85.48 & \underline{25.88} \\
    VB8Fusion  & \textbf{76.10} & \textbf{86.56} & 25.02 \\
    VB10Fusion & \underline{75.61} & \underline{85.95} & 25.19 \\
    VB12Fusion & 75.29 & 85.34 & \textbf{26.26} \\
    \bottomrule
    \end{tabular*}
    \label{10B_RSVQAxBEN_acc}
    \end{subtable}
\end{table}


% \begin{table}[b!]
%     \centering
%     \caption{Accuracy obtained by the different models on the RSVQAxBEN Dataset.}
%     \begin{tabularx}{\linewidth}{X X X X X X X X X X S[table-text-alignment=none]}
%     \toprule
%     Model & Global & Yes/No & YN1 & YN2 & YN3 & LC & LC0 & LC1 & {LC2} \\
%     \midrule
%     SkipRes & 69.92 & 80.02 &  83.29 & 78.91 & 71.27 & 20.68 & 19.38 & 18.82 & 25.01\\
%     Prompt-RSVQA & 75.40 & 86.07 & - & - & - & 26.56 & - & - & {W} \\
%     VB4layer & 73.06 & 83.86 & 85.44 & 83.30 & 77.05 & 20.40 & 18.15 & 19.80 & 26.96 \\
%     VB6layer & 73.88 & 84.58 & 86.22 & 84.01 & 77.83 & 21.66 & 19.88 & 20.65 & 27.93 \\
%     VB8layer & 73.43 & 84.37 & 86.05 & 83.64 & 77.75 & 20.07 & 18.02 & 19.61 & 25.86 \\
%     VB10layer & 74.19 & 85.13 & 86.55 & 84.69 & 79.24 & 20.82 & 19.39 & 20.12 & 25.79 \\
%     VB12layer & 75.07 & 85.47 & 86.95 & 84.81 & 79.91 & 24.33 & 24.22 & 23.22 & 27.34 \\
%     \bottomrule
%     \end{tabularx}
%     \label{RSVQAxBEN_acc}
% \end{table}

The results of the 10B RSVQAxBEN experiments are shown in \cref{10B_RSVQAxBEN_acc}.
From the table, we observe an improvement for all models compared to their RGB-trained counterparts.
Most of the observed performance increases can be justified by the improved LC accuracy.
An improved LC performance is expected, since some LC classes, such as different types of vegetation, greatly benefit from additional spectral information.
The smallest model, VB4Fusion, outperforms SkipRes (trained on RGB) by more than 5\% and slightly beats VB12Fusion trained on RGB.
The VB8Fusion model has the highest global accuracy, outperforming every other model, including Prompt-RSVQA trained on RGB RSVQAxBEN.
For VB12Fusion, the LC accuracy was already relatively high on RGB RSVQAxBEN.
Thus, it has the lowest improvement on the 10 bands dataset.  
Also, it is noteworthy that VB12Fusion has the second lowest global accuracy.
The relatively poor performance of VB12Fusion can be interpreted as a discrepancy between the RGB image feature representation and the 10 band feature representation, since VB12Fusion utilizes all pre-trained weights attained from ImageNet images.

%%%%%%%%%%%%%%%%%EXAMPLES
%%%%% RSVQAxBEN example

% \begin{table}[b!]
%     \centering
%     \includegraphics[]{graphics/visual_examples/S2A_MSIL2A_20170704T112111_47_33.png}
%     \caption{Example Results}
%     \begin{tabular*}{.5\linewidth}{l l}
%     \toprule
%     {Question} & {Are agricultural areas or artificial areas present?} \\
%     \midrule
%     GT & No \\
%     RGB Models  & {--} \\
%     VB4Fusion & Yes\\
%     VB8Fusion & Yes\\
%     VB12Fusion & Yes\\
%     10B Models &  {--} \\
%     VB4Fusion & Yes\\
%     VB8Fusion & Yes\\
%     VB12Fusion & Yes\\
%     \bottomrule
%     \end{tabular*}
%     \label{RSVQAxBEN_example1}
% \end{table}

% %%%%% RSVQAxBEN example

% \begin{table}[b!]
%     \centering
%     \includegraphics[]{graphics/visual_examples/S2A_MSIL2A_20170701T093031_59_2.png}
%     \caption{Example Results}
%     \begin{tabular*}{.5\linewidth}{l l}
%     \toprule
%     {Question} & {Which L3 classes are in the scene?} \\
%     \midrule
%     GT &  Coniferous Fores, Mixed Forest and Transitional Woodland/Shrub \\
%     RGB Models  & {--} \\
%     VB4Fusion & Broad-Leaved Forest\\
%     VB8Fusion & Broad-Leaved Forest and Transitional Woodland/Shrub\\
%     VB12Fusion & Broad-Leaved Forest and Transitional Woodland/Shrub\\
%     10B Models &  {--} \\
%     VB4Fusion & Coniferous Forest and Mixed Forest \\
%     VB8Fusion & Coniferous Forest and Mixed Forest \\
%     VB12Fusion & Broad-Leaved Forest\\
%     \bottomrule
%     \end{tabular*}
%     \label{RSVQAxBEN_example2}
% \end{table}

% %%%%% RSVQAxBEN example

% \begin{table}[b!]
%     \centering
%     \includegraphics[]{graphics/visual_examples/S2A_MSIL2A_20170613T101031_62_53.png}
%     \caption{Example Results}
%     \begin{tabular*}{.5\linewidth}{l l}
%     \toprule
%     {Question} & {Are there water bodies or wetlands?} \\
%     \midrule
%     GT & No \\
%     RGB Models  & {--} \\
%     VB4Fusion & No\\
%     VB8Fusion & No\\
%     VB12Fusion & Yes\\
%     10B Models &  {--} \\
%     VB4Fusion & No \\
%     VB8Fusion & No \\
%     VB12Fusion & No\\
%     \bottomrule
%     \end{tabular*}
%     \label{RSVQAxBEN_example3}
% \end{table}


% %%%%% LR EXAMPLE
% \begin{table}[b!]
%     \centering
%     \includegraphics[scale=0.5]{graphics/LR_example_312.png}
%     \caption{Example Results}
%     \begin{tabular*}{.5\linewidth}{l l}
%     \toprule
%     {Question} & {Is the number of Roads equal to the Commercial Buildings?} \\
%     \midrule
%     GT & No \\
%     VB4Fusion & No\\
%     VB8Fusion & No\\
%     VB12Fusion & No\\
%     \bottomrule
%     \end{tabular*}
%     \label{LR_RSVQA_example1}
% \end{table}

% %%%%% LR EXAMPLE

% \begin{table}[b!]
%     \centering
%     \includegraphics[scale=0.5]{graphics/LR_example_309.png}
%     \caption{Example Results}
%     \begin{tabular*}{.5\linewidth}{l l}
%     \toprule
%     {Question} & {Is a rectangular Grass area present?} \\
%     \midrule
%     GT & Yes \\
%     VB4Fusion & Yes \\
%     VB8Fusion & Yes \\
%     VB12Fusion & Yes \\
%     \bottomrule
%     \end{tabular*}
%     \label{LR_RSVQA_example2}
% \end{table}

% %%%%% LR EXAMPLE

% \begin{table}[b!]
%     \centering
%     \includegraphics[scale=0.5]{graphics/LR_example_227.png}
%     \caption{Example Results}
%     \begin{tabular*}{.5\linewidth}{l l}
%     \toprule
%     {Question} & {Is a small building present?} \\
%     \midrule
%     GT & Yes \\
%     VB4Fusion & Yes \\
%     VB8Fusion & Yes \\
%     VB12Fusion & Yes \\
%     \bottomrule
%     \end{tabular*}
%     \label{LR_RSVQA_example2}
% \end{table}



==> old_sections/introduction.tex <==
With advances in satellite technology, remote sensing (RS) data archives are rapidly growing, providing an unprecedented amount of images.
As a result, there has been an increased demand for systems that provide an intuitive interface to this wealth of Earth surface information.
For this purpose, visual question answering (VQA) has been introduced to the RS domain and has recently become an important research topic \citenum{RSVQA}.
VQA defines a framework that allows retrieval of use-case-specific information \citenum{VQA}.
By asking a free-form question to a selected image, the user can query various types of information without any need for computer vision-related expertise.

Most of the existing VQA architectures consist of three main modules: i) the feature extraction module; ii) the fusion module; and iii) the classification module.
The feature extraction module extracts high-level features for both input modalities (i.e., image and question text).
After encoding the input modalities, the fusion module is required to discover a cross-interaction between both features.
Since the model needs to select the relevant part of the image concerning the question, combining the features in a meaningful way is crucial.
Finally, the output of the fusion module is passed to the classification module to generate the natural language answer.
In the RS domain, relatively few VQA architectures were investigated \citenum{RSVQA,cross-modal,MutualAtt,three_class_heads,mcb_mutan_rs,Chappuis_2022_CVPR}.
In \citenum{RSVQA}, the feature extraction module applies a convolutional neural network (CNN) as an image encoder. The natural language encoder is based on the skip-thoughts \citenum{skip_thoughts} architecture, while the fusion module is a simple, non-learnable point-wise multiplication of the feature vectors.
In \citenum{MutualAtt}, a VGG-16 network \citenum{VGG_net} provides two kinds of visual features, a visual feature map extracted from the last convolutional layer and a visual feature vector derived from the final fully connected layer.
The language features are extracted by a gated-recurrent unit (GRU)\citenum{GRU}\,.
Both modality-specific representations are merged by the fusion module that leverages the more complex mutual-attention component.
In \citenum{mcb_mutan_rs}, the authors reveal the potential of an effective fusion module to build competitive RS VQA models.
This potential can already be seen in state-of-the-art CV-VQA architectures.
These architectures indicate that to fully utilize the information given by the image and the question, the model must learn their joint representation instead of statically combining the modality-specific representations.
In \citenum{cross-modal}, this knowledge is transferred to the RS VQA domain by introducing the first transformer-based architecture combined with an object detector pre-processor for the image features (called as \emph{CrossModal}).
The object detector is trained on the xView dataset \citenum{xView} to recognize identities like cars, houses, or ships.
In \citenum{Chappuis_2022_CVPR} a model, \emph{Prompt-RSVQA}, that takes advantage of the language transformer DistilBERT\citenum{distilBERT}, is proposed.
To this end, the feature extraction module projects the image into a word embedding space by passing through a multi-class classification network.
The image features encoded as words and the question text are merged in the transformer-based fusion module.
Both models provide promising results, guiding the motivation towards fusion modules that exploit transformer-based architectures.
However, the models presented lack generality.
As the CrossModal model from \citenum{cross-modal} focuses on objects, it could be challenging for the model to answer questions considering only Land Cover (LC) classes. 
% There are datasets that focus on LC-specific questions, such as the RSVQAxBEN \citenum{RSVQAxBEN} dataset.
% defined objects
The LC classes (e.g., water areas) are often not defined as objects in object-detection datasets such as xView.
In contrast, the model proposed in \citenum{Chappuis_2022_CVPR} extracts the LC information from a given image and only uses that class-level information to generate the visual feature vector.
Therefore, the model heavily exploits the presence of LC classes.
However, the model has the limitation that it lacks the ability to handle questions concerning objects or other low-level features not given by LC classes (e.g., questions included in the dataset proposed in \citenum{RSVQA}) and the relations among them.
However, these architectures provide reliable benchmarks for more general models.

To overcome these issues, in this paper, we present \emph{VBxFusion}, an architecture that leverages x multi-modal transformer layers of the VisualBERT \citenum{VisualBERT}\, model as fusion module.
Instead of applying an object detector, we utilize \emph{BoxExtractor}, a more general box extractor which does not overemphasize objects, within the visual feature extraction module.
The resulting boxes are fed into a ResNet \citenum{ResNet} to generate image tokens as embeddings of the extracted boxes.
For the text modality, a BertTokenizer \citenum{BERT} is used to tokenize the questions.
Our fusion module takes the modality-specific tokens as input and processes them with VisualBERT.
The classification module consists of a \gls{mlp} that generates a final vector representing the answer.
The proposed architecture is capable of handling all kinds of questions (e.g., concerning objects or LC classes).
The experimental results are obtained on large-scale RS VQA benchmark datasets\citenum{RSVQAxBEN,RSVQA}\,.
Furthermore, we analyze the importance of the utilized spectral bands by training the model on the same dataset with RGB and multispectral images.
We demonstrate the effectiveness of the multi-modal transformer compared to the architectures that use modality-specific feature combinations in the fusion module and compare the performance to the other more specific transformer models.
The results also show that including additional spectral bands significantly improves the performance.
To the best of our knowledge, this is the first study to consider multispectral RS VQA.
% It is worth noting that transformer-based architectures have a considerably higher computational complexity than the previous RS VQA models.
% Thus, we will also provide a detailed analysis of the trade-off between the VQA model complexity and accuracy. 

% \todo[inline]{Either do the trade-off analysis or change the sentence.}

The remaining sections are organized as follows; \cref{sec:method} will introduce the proposed architecture, including the feature extraction pipeline.
In \cref{sec:exp}, we will introduce the datasets for the experiments and analyze our results.
We will conclude our work in \cref{sec:con} and provide an outlook for future research directions.


==> old_sections/method.tex <==
\begin{figure}[tb!]
    \centering
    \includegraphics[width=.95\linewidth]{graphics/Model.png}
    \caption{A general overview of our proposed RS VQA model.
    Our model includes: i) a feature extraction module (\cref{feature_extraction_module}); ii) a fusion module (\cref{fusion_module}); and iii) a classification module (\cref{classification_module}).
    An RS image and a question about this image are considered as input.
    Inside the VisualBERT model, the modality-specific features get projected to a hidden dimension and concatenated afterwards.
    The concatenated features are then fed to $x$ Self-Attention Layers, providing an output for further processing in the classification module.
    The output of the classification module is a vector representing the final answer to the question.}
    \label{overview_model}
\end{figure}

In this section, we present the details of our proposed multi-modal fusion transformer.
The proposed architecture includes: i) a feature extraction module based on the BoxExtractor and the BertTokenizer; ii) a fusion module based on x multi-modal transformer layers of VisualBERT; and iii) a classification module consisting of an \gls{mlp} projection head. 
The general architecture overview is shown in \cref{overview_model}.
The details of each module are described in the following.

% TOOD: Discuss if we even need subsectiosn
\subsection{Feature Extraction Module}
\label{feature_extraction_module}
The feature extraction module aims to extract relevant features of the text and the vision modality independently from each other.
In the case of the vision modality, we utilize a simplified box extractor and a ResNet152\citenum{ResNet}\,.
The ResNet output is transformed with an \gls{mlp} layer into a suitable shape for the fusion module.
For the text modality, a pre-trained natural language processing tokenizer extracts the features of the questions.
To extract the image features, in CV it is common to guide the focus of a model to the relevant areas of the image \citenum{VisualBERT, BottomUp}.
For this reason, the state-of-the-art VQA models leverage an object detector to focus on important regions (i.e., objects).
For example, in VisualBERT\citenum{VisualBERT} a Faster R-CNN \citenum{FasterRCNN} backbone is used, to pre-process the image.
In the context of RS images, semantic segmentation is often applied to extract regions of interest (ROI), which may include specific pre-defined objects. 
Regarding the complexity of RS data, training a general semantic segmentation model capable of extracting general ROI requires a huge amount of labeled data.
Since labeling such an amount of data is costly, we propose \emph{BoxExtractor}.
BoxExtractor generates rectangular regions, boxes, that include any ROI without requiring labeled training data.

The image feature extraction pipeline is illustrated in
% Our visual feature extraction pipeline is depicted in
\cref{visual_feature_extraction}.
\begin{figure}[tb!]
    \centering
    \includegraphics[width=.9\linewidth]{graphics/image_features_extractor.png}
    \caption{The image feature extraction module takes an image as an input and outputs a feature map matrix. First, the box extractor creates the raw boxes from the input image, which has the sizes $n_{band} \times H_i^{'} \times W_i^{'}, i=1,...,n_{box}$. 
    These raw boxes are interpolated to the size $n_{band} \times H' \times W'$ and then fed into a ResNet152 network.
    The ResNet output (size $n_{box} \times K$) is then projected to an adjustable size with an \gls{mlp} layer.
    Here we choose $v$ as the visual embedding dimension of VisualBERT.}
    \label{visual_feature_extraction}
\end{figure}
To obtain the image features, we first create spatially interpolated rectangular regions of the image with our BoxExtractor. For this purpose, let $n_{\textrm{band}} \in \mathbb{N}$ be the number of spectral bands, $H, W \in \mathbb{N}$ the height and width of the images in the dataset, and $H', W' \in \mathbb{N}$ the height and width of the interpolated boxes.
Let $n_{\textrm{box}} \in \mathbb{N}$ be the number of boxes that BoxExtractor creates.
Then the function $B: \mathbb{R}^{ n_{\textrm{band}} \times H \times W} \to \mathbb{R}^{n_{\textrm{box}} \times n_{\textrm{band}} \times H' \times W'}$ maps an image $I$ to its boxes $B(I) = I^\prime$ in a non-deterministic way.
The non-determinism is observed because we first choose random start- and end-points for the height and the width of the boxes, $s_H^i, e_H^i \in \{0, 1, ..., H\}$, $s_H^i < e_H^i$ and $s_W^i, e_W^i \in \{0, 1, ..., W\}$, $s_W^i < e_W^i$, for $i \in \{1, ..., n_{\textrm{box}}\}$. In the second step, a vector of boxes is created.
We control the distance between the start- and endpoints (e.g., $e_H^i - s_H^i$) to guarantee a minimum amount of information in each box.
To this end, we set
\begin{equation}
    \text{min}_H \leq e_H^i - s_H^i 
\end{equation}
and
\begin{equation}
    \text{min}_W \leq e_W^i - s_W^i,
\end{equation}
for $i = 1, ..., n_{\textrm{box}}$, where $\text{min}_H, \text{min}_W$ are hyperparameters.
The resulting boxes are resized equally to $H'$ and $W'$ by bicubic interpolation. 

Next, we stack the image boxes and pass them to a pre-trained ResNet152\citenum{ResNet}\, network.
Finally, we must transform the output into a suitable shape for the fusion module.
We reshape the features and keep the number of boxes as the first dimension, whereas the second dimension is given by flattening the remaining directions, resulting in a matrix.
The matrix is fed into a linear layer to project its size to $n_{\textrm{box}} \times v$, where $v \in \mathbb{N}$ is the so-called visual embedding dimension of the VisualBERT\citenum{VisualBERT} model (i.e., the required input dimension for the vision modality).
Note that, except for the last linear layer, the image feature extraction module is frozen and may be applied as a pre-processing step.
% In the actual code, the linear layer is shifted to the fusion model. % <- irrelevant for the paper
% In the case of 10 bands, $b=10$, we have to resize the spectral bands before the box extraction to have all bands in the same resolution. % <- Implementation detail that is 'well-known' when working with multi-spectral data; doesn't fit the narrative here

To extract the language features from the question, we translate each question into tokens.
These tokens are a mapping of the words to a numerical value.
To achieve this and to be aligned with the original VisualBERT\citenum{VisualBERT} model, we utilize a frozen BertTokenizer\citenum{BERT}\,.
Both the visual and the language features are jointly processed to extract their implicit knowledge in the next step.

\subsection{Fusion Module}
\label{fusion_module}
Our proposed transformer-based fusion module jointly learns the alignment between the image and text modality.
To learn the joint alignment, we leverage VisualBERT \citenum{VisualBERT}.
VisualBERT represents the extension of the language transformer BERT with the vision modality.
VisualBERT first projects the image features into a suitable shape to concatenate the projected image features with the language modality.
The concatenated features are then fed to the BERT transformer layers.
The output is given by pooling the last hidden state.
The resulting vector is further processed in the classification module.
To summarize the forward procedure, VisualBERT fuses the vision and language modality and feeds them into the BERT architecture, representing a natural extension of BERT to multiple modalities.
Additionally, VisualBERT shows competitive results on VQA benchmark datasets and is thus well suited as a starting point for multi-modal fusion transformers in RS VQA.

In contrary to the previous RS VQA models that statically combine both modalities in a non-learnable way, our model learns a joint representation.
% Our proposed RS VQA architecture contraries the previous RS VQA models, which combine both modalities in a non-learnable way.
Note that our approach differs from \citenum{Chappuis_2022_CVPR} as they apply a transformer based on the language modality only.
In contrast to the model proposed in \citenum{cross-modal}, we apply exclusively multi-modal self-attention instead of a mixture of single- and multi-modal self-attention. 

\subsection{Classification Module}
\label{classification_module}

The task of the classification module is to create a classification vector representing the prediction for the specific answers.
Following \citenum{RSVQA}, we utilize an \gls{mlp} as a classification module.
The \gls{mlp} consists of three layers, where the last layer has the dimension of the considered answer set.
The final answer is then obtained by selecting the largest activation of the output vector.
% Remark that the answers are declining sorted in a vector by their occurrence frequency, and the position of the answers in this sorted vector is the corresponding entries of the classification vector. % <= Also not relevant for this section

